Sense and sensitivity of double beta decay experiments

The search for neutrinoless double beta decay is a very active field in which the number of proposals for next-generation experiments has proliferated. In this paper we attempt to address both the sense and the sensitivity of such proposals. Sensitivity comes first, by means of proposing a simple and unambiguous statistical recipe to derive the sensitivity to a putative Majorana neutrino mass, m_bb. In order to make sense of how the different experimental approaches compare, we apply this recipe to a selection of proposals, comparing the resulting sensitivities. We also propose a "physics-motivated range" (PMR) of the nuclear matrix elements as a unifying criterium between the different nuclear models. The expected performance of the proposals is parametrized in terms of only four numbers: energy resolution, background rate (per unit time, isotope mass and energy), detection efficiency, and bb isotope mass. For each proposal, both a reference and an optimistic scenario for the experimental performance are studied. In the reference scenario we find that all the proposals will be able to partially explore the degenerate spectrum, without fully covering it, although four of them (KamLAND-Zen, CUORE, NEXT and EXO) will approach the 50 meV boundary. In the optimistic scenario, we find that CUORE and the xenon-based proposals (KamLAND-Zen, EXO and NEXT) will explore a significant fraction of the inverse hierarchy, with NEXT covering it almost fully. For the long term future, we argue that Xe-based experiments may provide the best case for a 1-ton scale experiment, given the potentially very low backgrounds achievable and the expected scalability to large isotope masses.

==> src/Resolution.tex <==
\subsection{The sensitivity of next-generation experiments}\label{subsec:results_resolution}

\begin{table}[t!]
\begin{center}
\begin{tabular}{l D{.}{.}{-1} D{.}{.}{-1} D{.}{.}{-1} D{.}{.}{-1} D{.}{.}{-1}}
\hline\hline
\multirow{2}{*}{Experiment} & \multicolumn{5}{c}{ \mbb\ (meV)} \\ \cline{2-6}
 & \multicolumn{1}{c}{$c=10^{-1}$} & \multicolumn{1}{c}{$c=10^{-2}$} & \multicolumn{1}{c}{$c=10^{-3}$} & \multicolumn{1}{c}{$c=10^{-4}$} & \multicolumn{1}{c}{$c=10^{-5}$}\\ \hline \noalign{\smallskip}
CUORE          &  93 &  {\bf 54} & 34 & 25 & 00\\
EXO            & 244 &   139 & {\bf 80} & 49 & 00\\
GERDA & 156 &  {\bf 91} & 58 & 41 & 00\\
KamLAND-Zen    & 300 &  169 & 97 & {\bf 57} & 00\\
NEXT           &  257 &  147 & 87 & {\bf 58} & 00\\
SNO+           & 297 &  168 & {\bf 96} & 57 & 00\\
SuperNEMO      & 328 &  186 & 107 & {\bf 64} & 00\\
\hline\hline
\end{tabular}
\end{center}
\caption{Large exposure \mbb\ sensitivity (for $Mt= 10^{3}\ \kgy$ and at 90\% CL) of different \bbonu\ experiments.  The background rate $c$ is expressed in \ckky. The numbers in bold face represent the expected background rate
in the (C) scenario of the different proposals.}
\label{tab.sensi}
\end{table}%

Table \ref{tab.sensi} gives the sensitivity for large exposure of ($10^3\ \kgy$), for all experiments and for four different background rate assumptions. In the background rate characterizing current \bbonu\ experiments, $c\sim 10^{-1}\ \ckky$, only CUORE  would have a (weak) case, reaching \mbb\ sensitivities below 100 meV at 90\% CL with a 5 years run. With a one order of magnitude background rate suppression, $c=10^{-2}\ \ckky$, GERDA would reach 90 meV at 90\% CL and CUORE would almost fully explore the inverted hierarchy (down to 54 meV at 90\% CL). For background rates at the $10^{-3}\ \ckky$ level, CUORE would probe the inverted hierarchy (down to \mbb\ $\sim 34$ meV), GERDA would approach the frontier of the degenerate spectrum, while EXO, NEXT and SNO+, would just drop the 100 meV limit. Finally, for even lower background rates, $c=10^{-4}\ \ckky$, CUORE would almost fullt explore the inverted hierarchy, GERDA would start to scan it and the rest of the proposals would cover the degenerate spectrum. 

Consider now the numbers in bold face, which reflect the background rate in the (C) scenario which will probably be the most likely one in the next decade. Here we find CUORE, Kamland-ZEN and NEXT close but not quite reaching the 50 meV landmark, with the rest of the proposals covering the region between 64 meV (SuperNEMO) and 96 meV (SNO+). It follows that the ``next-generation'' of experiments, that will run over the next ten years or so, with masses in the vicinity of 100 kg, will, at best, explore the degenerate spectrum. 

